Inference from Sampling with Response Probabilities Estimated via Calibration

A solution to control for nonresponse bias consists of multiplying the design weights of respondents by the inverse of estimated response probabilities to compensate for the nonrespondents. Maximum likelihood and calibration are two approaches that can be applied to obtain estimated response probabilities. We consider a common framework in which these approaches can be compared. We develop an asymptotic study of the behavior of the resulting estimator when calibration is applied. A logistic regression model for the response probabilities is postulated. Missing at random and unclustered data are supposed. Three main contributions of this work are: 1) we show that the estimators with the response probabilities estimated via calibration are asymptotically equivalent to unbiased estimators and that a gain in efficiency is obtained when estimating the response probabilities via calibration as compared to the estimator with the true response probabilities, 2) we show that the estimators with the response probabilities estimated via calibration are doubly robust to model misspecification and explain why double robustness is not guaranteed when maximum likelihood is applied, and 3) we discuss and illustrate problems related to response probabilities estimation, namely existence of a solution to the estimating equations, problems of convergence, and extreme weights. We explain and illustrate why the first aforementioned problem is more likely with calibration than with maximum likelihood estimation. We present the results of a simulation study in order to illustrate these elements.

==> figs/scenario1_results.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 14 15:00:27 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
 & RB & RRVAR \\
  \hline
HT & $-1.26 \times 10^{-5}$             & $3.20 \times 10^{-2}$ \\
p & \alert<1>{$1.03 \times 10^{-3}$}    & \alert<2>{$1.33 \times 10^{-1}$} \\
na\"if & \alert<3>{$-1.43 \times 10^{-1}$}& $4.41 \times 10^{-2}$ \\
mle & \alert<1>{$1.51 \times 10^{-3}$}  & \alert<2>{$8.11 \times 10^{-2}$} \\
calU & \alert<1>{$-2.89 \times 10^{-4}$} & \alert<2>{$4.46 \times 10^{-2}$} \\
calS & \alert<1>{$-2.22 \times 10^{-4}$} & \alert<2>{$4.88 \times 10^{-2}$} \\
   \hline
\end{tabular}
\end{table}


==> figs/scenario2_results.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 14 15:29:29 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & 1 & 2 & 3 \\
  \hline
mle & $9.58 \times 10^{-2}$ & $8.11 \times 10^{-2}$ & $6.54 \times 10^{-2}$ \\
calU & \alert<1-2>{$9.11 \times 10^{-2}$} & \alert<1-3>{$4.46 \times 10^{-2}$} & \alert<1-3>{$3.58 \times 10^{-3}$} \\
calS & \alert<1-2>{$8.99 \times 10^{-2}$} & \alert<1-3>{$4.88 \times 10^{-2}$} & \alert<1-3>{$1.96 \times 10^{-2}$} \\
   \hline
\end{tabular}
\end{table}


==> figs/scenario3_results1.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 14 15:50:57 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
 & RRVAR & rate cal/estim eqn \\
  \hline
mle & $9.35 \times 10^{-2}$ & \alert<4>{0.9999} \\
calU & \alert<1>{$4.47 \times 10^{-2}$} & \alert<2-3>{0.2133} \\
calS & \alert<1>{$9.71 \times 10^{-2}$} & \alert<2-3>{0.1591} \\
   \hline
\end{tabular}
\end{table}


==> figs/scenario4_results.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 14 16:02:53 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
 & RB & RRVAR \\
  \hline
HT & $-1.40 \times 10^{-4}$ & $3.20 \times 10^{-2}$ \\
p & \alert<1->{$3.06 \times 10^{-3}$} & $1.81 \times 10^{-1}$ \\
na\"if & $-1.76 \times 10^{-1}$ & $4.29 \times 10^{-2}$ \\
mle & \alert<2->{$-1.13 \times 10^{-1}$} & $8.90 \times 10^{-2}$ \\
calU & \alert<1->{$2.30 \times 10^{-3}$} & $5.33 \times 10^{-2}$ \\
calS & \alert<1->{$2.73 \times 10^{-3}$} & $5.72 \times 10^{-2}$ \\
   \hline
\end{tabular}
\end{table}


==> figs/table_tot_pois.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Jan 13 14:05:15 2022
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrr}
  \hline
 & RB & RRVAR & RB & RRVAR & RB & RRVAR \\ 
  \hline
ybar\_ht & $-5.95 \times 10^{-3}$ & $1.19 \times 10^{-1}$ & $-5.79 \times 10^{-3}$ & $1.11 \times 10^{-1}$ & $-7.06 \times 10^{-3}$ & $1.11 \times 10^{-1}$ \\ 
  ybar\_p & $-7.80 \times 10^{-3}$ & $1.27 \times 10^{-1}$ & $-6.89 \times 10^{-3}$ & $1.19 \times 10^{-1}$ & $-8.60 \times 10^{-3}$ & $1.19 \times 10^{-1}$ \\ 
  ybar\_p\_mle & $-5.26 \times 10^{-3}$ & $1.21 \times 10^{-1}$ & $-4.99 \times 10^{-3}$ & $1.13 \times 10^{-1}$ & $-6.44 \times 10^{-3}$ & $1.13 \times 10^{-1}$ \\ 
  ybar\_p\_mlepi & $-5.90 \times 10^{-3}$ & $1.19 \times 10^{-1}$ & $-5.71 \times 10^{-3}$ & $1.12 \times 10^{-1}$ & $-7.50 \times 10^{-3}$ & $1.12 \times 10^{-1}$ \\ 
  ybar\_p\_calU & $1.55 \times 10^{-3}$ & $2.78 \times 10^{-2}$ & $1.88 \times 10^{-3}$ & $3.04 \times 10^{-2}$ & $2.08 \times 10^{-3}$ & $3.66 \times 10^{-2}$ \\ 
  ybar\_p\_calS & $-5.92 \times 10^{-3}$ & $1.19 \times 10^{-1}$ & $-5.70 \times 10^{-3}$ & $1.12 \times 10^{-1}$ & $-7.48 \times 10^{-3}$ & $1.12 \times 10^{-1}$ \\ 
   \hline
\end{tabular}
\end{table}


==> figs/table_tot_srs.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Jan 13 13:57:55 2022
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrr}
  \hline
 & RB & RRVAR & RB & RRVAR & RB & RRVAR \\ 
  \hline
ybar\_ht & $-3.27 \times 10^{-5}$ & $2.46 \times 10^{-2}$ & $-3.48 \times 10^{-4}$ & $2.30 \times 10^{-2}$ & $2.46 \times 10^{-4}$ & $2.41 \times 10^{-2}$ \\ 
  ybar\_p & $9.10 \times 10^{-5}$ & $4.99 \times 10^{-2}$ & $2.10 \times 10^{-4}$ & $5.00 \times 10^{-2}$ & $8.47 \times 10^{-4}$ & $5.19 \times 10^{-2}$ \\ 
  ybar\_p\_mle & $2.52 \times 10^{-5}$ & $2.62 \times 10^{-2}$ & $-5.51 \times 10^{-4}$ & $2.61 \times 10^{-2}$ & $-2.06 \times 10^{-4}$ & $2.79 \times 10^{-2}$ \\ 
  ybar\_p\_mlepi & $2.33 \times 10^{-5}$ & $2.62 \times 10^{-2}$ & $-5.51 \times 10^{-4}$ & $2.60 \times 10^{-2}$ & $-2.06 \times 10^{-4}$ & $2.79 \times 10^{-2}$ \\ 
  ybar\_p\_calU & $1.12 \times 10^{-4}$ & $2.14 \times 10^{-2}$ & $-4.34 \times 10^{-4}$ & $2.52 \times 10^{-2}$ & $-2.21 \times 10^{-5}$ & $2.95 \times 10^{-2}$ \\ 
  ybar\_p\_calS & $1.53 \times 10^{-4}$ & $2.63 \times 10^{-2}$ & $-4.37 \times 10^{-4}$ & $2.55 \times 10^{-2}$ & $-1.31 \times 10^{-4}$ & $2.71 \times 10^{-2}$ \\ 
   \hline
\end{tabular}
\end{table}


==> figs/table_tot_srs_pois_clean.tex <==
% latex table modified from tables generated in R 4.1.2 by xtable 1.8-4 package
% Thu Jan 13 13:57:55 2022
\begin{table}[ht]
\caption{Relative bias (RB) and relative root variance (RRVAR) for six estimators, three populations, and two sampling designs.\label{table:total}}
\begin{center}
\begin{tabular}{rrrrrrr}
  \toprule
 & \multicolumn{6}{c}{Simple Random Sampling}\\
 \cmidrule{2-7}
 & \multicolumn{2}{c}{Population 1}&\multicolumn{2}{c}{Population 2}&\multicolumn{2}{c}{Population 3}\\
  & \multicolumn{2}{c}{$\rho = 0.6$}&\multicolumn{2}{c}{$\rho = 0.3$}&\multicolumn{2}{c}{$\rho = 0$}\\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & RB & RRVAR & RB & RRVAR & RB & RRVAR \\
  & $(\times 10^{-4})$ & $(\times 10^{-2})$ & $(\times 10^{-4})$ & $(\times 10^{-2})$ & $(\times 10^{-4})$ & $(\times 10^{-2})$ \\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
HT          & $-0.33$   & $2.46 $ & $-3.48 $ & $2.30 $ & $2.46 $ & $2.41$ \\
$p$         & $0.91$    & $4.99 $ & $2.10 $  & $5.00 $ & $8.47 $ & $5.19$ \\
mle, $1$    & $0.25 $   & $2.62 $ & $-5.51 $ & $2.61 $ & $-2.06$ & $2.79$ \\
mle, $1/\pi$& $0.23$    & $2.62 $ & $-5.51 $ & $2.60 $ & $-2.06$ & $2.79$ \\
cal, $U$    & $1.12 $   & $2.14 $ & $-4.34 $ & $2.52 $ & $-0.22$ & $2.95$ \\
cal, $S$    & $1.53$    & $2.63 $ & $-4.37 $ & $2.55 $ & $-1.31$ & $2.71$ \\
\cmidrule{2-7}
 & \multicolumn{6}{c}{Poisson Sampling}\\
 \cmidrule{2-7}
  & \multicolumn{2}{c}{Population 1}&\multicolumn{2}{c}{Population 2}&\multicolumn{2}{c}{Population 3}\\
  & \multicolumn{2}{c}{$\rho = 0.6$}&\multicolumn{2}{c}{$\rho = 0.3$}&\multicolumn{2}{c}{$\rho = 0$}\\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & RB & RRVAR & RB & RRVAR & RB & RRVAR \\
 & $(\times 10^{-3})$ & $(\times 10^{-1})$ & $(\times 10^{-3})$ & $(\times 10^{-1})$ & $(\times 10^{-3})$ & $(\times 10^{-1})$ \\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
HT          & $-5.95 $ & $1.19$ & $-5.79 $ & $1.11$ & $-7.06$ & $1.11$ \\
$p$         & $-7.80 $ & $1.27$ & $-6.89 $ & $1.19$ & $-8.60$ & $1.19$ \\
mle, $1$    & $-5.26 $ & $1.21$ & $-4.99 $ & $1.13$ & $-6.44$ & $1.13$ \\
mle, $1/\pi$& $-5.90 $ & $1.19$ & $-5.71 $ & $1.12$ & $-7.50$ & $1.12$ \\
cal, $U$    &  $1.55 $ & $0.28$ & $1.88  $ & $0.30$ & $2.08 $ & $3.66$ \\
cal, $S$    & $-5.92 $ & $1.19$ & $-5.70 $ & $1.12$ & $-7.48$ & $1.12$ \\
   \bottomrule
\end{tabular}
\end{center}
\end{table}


==> figs/table_var.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 17 20:46:01 2022
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrrrr}
  \toprule
 & \multicolumn{9}{c}{Simple Random Sampling}\\
 \cmidrule{2-10}
 & \multicolumn{3}{c}{Population 1}&\multicolumn{3}{c}{Population 2}&\multicolumn{3}{c}{Population 3}\\
  & \multicolumn{3}{c}{$\rho = 0.6$}&\multicolumn{3}{c}{$\rho = 0.3$}&\multicolumn{3}{c}{$\rho = 0$}\\
   \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 & RB & Length & CR & RB & Length & CR & RB & Length & CR \\
  \hline
ybar\_p\_mle & 0.02 & 410 & 0.95 & -0.18 & 372 & 0.90 & -0.21 & 394 & 0.88 \\
  ybar\_p\_mlepi & 0.02 & 410 & 0.95 & -0.18 & 372 & 0.90 & -0.21 & 394 & 0.88 \\
  ybar\_p\_calU & -0.04 & 323 & 0.94 & -0.07 & 385 & 0.93 & -0.21 & 420 & 0.91 \\
  ybar\_p\_calS & 0.02 & 410 & 0.95 & -0.10 & 382 & 0.93 & -0.12 & 404 & 0.92 \\
  ybar\_p\_mle.1 & 0.10 & 1954 & 0.95 & 0.05 & 1778 & 0.93 & 0.05 & 1788 & 0.92 \\
  ybar\_p\_mlepi.1 & 0.13 & 1948 & 0.95 & 0.02 & 1809 & 0.95 & 0.02 & 1825 & 0.95 \\
  ybar\_p\_calU.1 & -0.13 & 391 & 0.92 & -0.05 & 449 & 0.93 & -0.09 & 510 & 0.90 \\
  ybar\_p\_calS.1 & 0.13 & 1948 & 0.95 & 0.03 & 1806 & 0.95 & 0.03 & 1823 & 0.95 \\
   \hline
\end{tabular}
\end{table}


==> figs/table_var_clean.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 17 20:46:01 2022
\begin{table}[ht]
\caption{Relative bias (RB) of the variance estimator, mean length of the 95\% confidence interval, and actual coverage of this interval for four NWA estimators.\label{table:variance}}
\begin{center}
\begin{tabular}{rrrrrrrrrrrrr}
  \toprule
 & \multicolumn{9}{c}{Simple Random Sampling}\\
 \cmidrule{2-10}
 & \multicolumn{3}{c}{Population 1}&\multicolumn{3}{c}{Population 2}&\multicolumn{3}{c}{Population 3}\\
  & \multicolumn{3}{c}{$\rho = 0.6$}&\multicolumn{3}{c}{$\rho = 0.3$}&\multicolumn{3}{c}{$\rho = 0$}\\
   \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 &    & \multicolumn{2}{c}{95\% CI} &    & \multicolumn{2}{c}{95\% CI}&    & \multicolumn{2}{c}{95\% CI} \\
 & RB & Length & CR & RB & Length & CR & RB & Length & CR \\
   \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
mle, $1$    & 0.02 & 410 & 0.95 & -0.18 & 372 & 0.90 & -0.21 & 394 & 0.88 \\
mle, $1/\pi$& 0.02 & 410 & 0.95 & -0.18 & 372 & 0.90 & -0.21 & 394 & 0.88 \\
cal, $U$    &-0.04 & 323 & 0.94 & -0.07 & 385 & 0.93 & -0.21 & 420 & 0.91 \\
cal, $S$    & 0.02 & 410 & 0.95 & -0.10 & 382 & 0.93 & -0.12 & 404 & 0.92 \\
\cmidrule{2-10}
 & \multicolumn{9}{c}{Poisson Sampling}\\
 \cmidrule{2-10}
 & \multicolumn{3}{c}{Population 1}&\multicolumn{3}{c}{Population 2}&\multicolumn{3}{c}{Population 3}\\
  & \multicolumn{3}{c}{$\rho = 0.6$}&\multicolumn{3}{c}{$\rho = 0.3$}&\multicolumn{3}{c}{$\rho = 0$}\\
   \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 &    & \multicolumn{2}{c}{95\% CI} &    & \multicolumn{2}{c}{95\% CI}&    & \multicolumn{2}{c}{95\% CI} \\
 & RB & Length & CR & RB & Length & CR & RB & Length & CR \\
   \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
mle, $1$    & 0.10 & 1954 & 0.95 & 0.05 & 1778 & 0.93 & 0.05 & 1788 & 0.92 \\
mle, $1/\pi$& 0.13 & 1948 & 0.95 & 0.02 & 1809 & 0.95 & 0.02 & 1825 & 0.95 \\
cal, $U$    & -0.13& 391 & 0.92 & -0.05 & 449 & 0.93 & -0.09 & 510 & 0.90 \\
cal, $S$    & 0.13 & 1948 & 0.95 & 0.03 & 1806 & 0.95 & 0.03 & 1823 & 0.95 \\
   \bottomrule
\end{tabular}
\end{center}
\end{table}


==> figs/table_weights.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Jan 18 09:13:46 2022
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \toprule
 & \multicolumn{6}{c}{Simple Random Sampling}\\
 \cmidrule{2-7}
 & \multicolumn{1}{c}{Population 1}&\multicolumn{1}{c}{Population 2}&\multicolumn{1}{c}{Population 3}\\
  & \multicolumn{1}{c}{$\rho = 0.6$}&\multicolumn{1}{c}{$\rho = 0.3$}&\multicolumn{1}{c}{$\rho = 0$}\\
   \cmidrule(lr){2}\cmidrule(lr){3}\cmidrule(lr){4}
ybar\_p & 16.7 & 16.7 & 16.7 \\
  ybar\_p\_mle & 18.2 & 17.8 & 19.1 \\
  ybar\_p\_mlepi & 19.6 & 17.8 & 19.1 \\
  ybar\_p\_calU & 18.0 & 17.9 & 18.3 \\
  ybar\_p\_calS & 18.0 & 17.6 & 17.9 \\
  ybar\_p.1 & 45.4 & 46.0 & 55.5 \\
  ybar\_p\_mle.1 & 51.0 & 45.5 & 53.8 \\
  ybar\_p\_mlepi.1 & 51.6 & 47.2 & 55.5 \\
  ybar\_p\_calU.1 & 67.9 & 62.7 & 71.2 \\
  ybar\_p\_calS.1 & 51.4 & 46.8 & 54.9 \\
   \hline
\end{tabular}
\end{table}


==> figs/table_weights_clean.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Jan 18 09:13:46 2022
\begin{table}[ht]
\caption{Maximum weight over $L=10'000$ simulations for five estimators, three populations, and two sampling designs.\label{table:weights}}
\begin{center}
\begin{tabular}{rccc}
  \toprule
 & \multicolumn{3}{c}{Simple Random Sampling}\\
 \cmidrule{2-4}
 & \multicolumn{1}{c}{Population 1}&\multicolumn{1}{c}{Population 2}&\multicolumn{1}{c}{Population 3}\\
  & \multicolumn{1}{c}{$\rho = 0.6$}&\multicolumn{1}{c}{$\rho = 0.3$}&\multicolumn{1}{c}{$\rho = 0$}\\
   \cmidrule{2-4}%\cmidrule{3}\cmidrule{4}
$p$         & 16.7 & 16.7 & 16.7 \\
mle, $1$    & 18.2 & 17.8 & 19.1 \\
mle, $1/\pi$& 19.6 & 17.8 & 19.1 \\
cal, $U$    & 18.0 & 17.9 & 18.3 \\
cal, $S$    & 18.0 & 17.6 & 17.9 \\
    \cmidrule{2-4}
 & \multicolumn{3}{c}{Poisson Sampling}\\
 \cmidrule{2-4}
 & \multicolumn{1}{c}{Population 1}&\multicolumn{1}{c}{Population 2}&\multicolumn{1}{c}{Population 3}\\
  & \multicolumn{1}{c}{$\rho = 0.6$}&\multicolumn{1}{c}{$\rho = 0.3$}&\multicolumn{1}{c}{$\rho = 0$}\\
  \cmidrule{2-4}
    $p$     & 45.4 & 46.0 & 55.5 \\
mle, $1$    & 51.0 & 45.5 & 53.8 \\
mle, $1/\pi$& 51.6 & 47.2 & 55.5 \\
cal, $U$    & 67.9 & 62.7 & 71.2 \\
cal, $S$    & 51.4 & 46.8 & 54.9 \\
   \bottomrule
\end{tabular}
\end{center}
\end{table}

